Producing a BOSS-CMASS sample with DES imaging

We present a sample of galaxies with the Dark Energy Survey (DES) photometry that replicates the properties of the BOSS CMASS sample. The CMASS galaxy sample has been well characterized by the Sloan Digital Sky Survey (SDSS) collaboration and was used to obtain the most powerful redshift-space galaxy clustering measurements to date. A joint analysis of redshift-space distortions (such as those probed by CMASS from SDSS) and a galaxy-galaxy lensing measurement for an equivalent sample from DES can provide powerful cosmological constraints. Unfortunately, the DES and SDSS-BOSS footprints have only minimal overlap, primarily on the celestial equator near the SDSS Stripe 82 region. Using this overlap, we build a robust Bayesian model to select CMASS-like galaxies in the remainder of the DES footprint. The newly defined DES-CMASS (DMASS) sample consists of 117,293 effective galaxies covering $1,244 {\rm deg}^2$. Through various validation tests, we show that the DMASS sample selected by this model matches well with the BOSS CMASS sample, specifically in the South Galactic cap (SGC) region that includes Stripe 82. Combining measurements of the angular correlation function and the clustering-z distribution of DMASS, we constrain the difference in mean galaxy bias and mean redshift between the BOSS CMASS and DMASS samples to be $\Delta b = 0.010^{+0.045}_{-0.052}$ and $\Delta z = \left( 3.46^{+5.48}_{-5.55} \right) \times 10^{-3}$ for the SGC portion of CMASS, and $\Delta b = 0.044^{+0.044}_{-0.043} $ and $\Delta z= ( 3.51^{+4.93}_{-5.91}) \times 10^{-3}$ for the full CMASS sample. These values indicate that the mean bias of galaxies and mean redshift in the DMASS sample is consistent with both CMASS samples within $1\sigma$.

==> Makefile <==
texfile := main
outputpdf := Lee_et_al_Producing_a_BOSS-CMASS_sample_with_DES_imaging.pdf

all:
	pdflatex ${texfile}
	bibtex ${texfile}
	bibtex ${texfile}
	pdflatex ${texfile}
	pdflatex ${texfile}
	pdflatex ${texfile}
	cp ${texfile}.pdf ${outputpdf}

bib: 
	bibtex ${texfile}
	bibtex ${texfile}

pdf: 
	pdflatex ${texfile}
	pdflatex ${texfile}

clean:
	rm -f \
	${texfile}.dvi \
	${texfile}.pdf \
	${texfile}.aux \
	${texfile}.bbl \
	${texfile}.blg \
	${texfile}.toc \
	${texfile}.log


==> authorlist <==
Lastname,Firstname,Email,Authorname,JoinedAsBuilder,Affiliation,ORCID
Lee,Sujeong,lee.5922@osu.edu,S.~Lee,False,"Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA",
Lee,Sujeong,lee.5922@osu.edu,S.~Lee,False,"Department of Physics, The Ohio State University, Columbus, OH 43210, USA",
Choi,Ami,choi.1442@osu.edu,A.~Choi,False,"Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA",
Davis,Christopher,cpd@stanford.edu,C.~Davis,False,"Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA",
Eifler,Tim,timeifler@gmail.com,T.~F.~Eifler,False,"Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA",0000-0002-1894-3301
Eifler,Tim,timeifler@gmail.com,T.~F.~Eifler,False,"Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA",0000-0002-1894-3301
Honscheid,Klaus,kh@fnal.gov,K.~Honscheid,False,"Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA",
Honscheid,Klaus,kh@fnal.gov,K.~Honscheid,False,"Department of Physics, The Ohio State University, Columbus, OH 43210, USA",
Huff,Eric,eric.m.huff@jpl.nasa.gov,E.~M.~Huff,False,"Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA",0000-0002-9378-3424
MacCrann,Niall,maccrann.2@osu.edu,N.~MacCrann,False,"Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA",
MacCrann,Niall,maccrann.2@osu.edu,N.~MacCrann,False,"Department of Physics, The Ohio State University, Columbus, OH 43210, USA",
Ross,Ashley,ashley.jacob.ross@gmail.com,A.~J.~Ross,False,"Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA",0000-0002-7522-9083
Troxel,Michael A.,michael.a.troxel@gmail.com,M.~A.~Troxel,False,"Department of Physics, Duke University Durham, NC 27708, USA",
Annis,James,annis@fnal.gov,J.~Annis,True,"Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA",0000-0002-0609-3987
Avila,Santiago,santiagoavilaperez@gmail.com,S.~Avila,True,"Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain",
Brooks,David,david.brooks@ucl.ac.uk,D.~Brooks,True,"Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK",
Carnero Rosell,Aurelio,aurelio.crosell@gmail.com,A.~Carnero~Rosell,True,"Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain",0000-0003-3044-5150
Carnero Rosell,Aurelio,aurelio.crosell@gmail.com,A.~Carnero~Rosell,True,"Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil",0000-0003-3044-5150
Carrasco Kind,Matias,mcarras2@illinois.edu,M.~Carrasco~Kind,True,"Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA",0000-0002-4802-3194
Carrasco Kind,Matias,mcarras2@illinois.edu,M.~Carrasco~Kind,True,"National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA",0000-0002-4802-3194
Carretero,Jorge,jorgecarreteropalacios@gmail.com,J.~Carretero,True,"Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain",0000-0002-3130-0204
Cawthon,Ross,rcawthon@oddjob.uchicago.edu,R.~Cawthon,True,"Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390",
da Costa,Luiz,ldacosta@fnal.gov,L.~N.~da Costa,True,"Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil",
da Costa,Luiz,ldacosta@fnal.gov,L.~N.~da Costa,True,"Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil",
De Vicente,Juan,juan.vicente@ciemat.es,J.~De~Vicente,True,"Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain",0000-0001-8318-6813
Desai,Shantanu,shntn05@gmail.com,S.~Desai,True,"Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India",0000-0002-0466-3288
Flaugher,Brenna,brenna@fnal.gov,B.~Flaugher,True,"Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA",
Fosalba,Pablo,fosalba@gmail.com,P.~Fosalba,True,"Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain",
Fosalba,Pablo,fosalba@gmail.com,P.~Fosalba,True,"Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain",
Garcia-Bellido,Juan,juan.garciabellido@uam.es,J.~Garc\'ia-Bellido,True,"Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain",0000-0002-9370-8360
Gaztanaga,Enrique,gaztanaga@gmail.com,E.~Gaztanaga,True,"Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain",
Gaztanaga,Enrique,gaztanaga@gmail.com,E.~Gaztanaga,True,"Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain",
Gerdes,David,gerdes@umich.edu,D.~W.~Gerdes,True,"Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA",0000-0001-6942-2736
Gerdes,David,gerdes@umich.edu,D.~W.~Gerdes,True,"Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA",0000-0001-6942-2736
Gruen,Daniel,dgruen@stanford.edu,D.~Gruen,True,"Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA",
Gruen,Daniel,dgruen@stanford.edu,D.~Gruen,True,"Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA",
Gruen,Daniel,dgruen@stanford.edu,D.~Gruen,True,"SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA",
Gruendl,Robert,gruendl@illinois.edu,R.~A.~Gruendl,True,"Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA",
Gruendl,Robert,gruendl@illinois.edu,R.~A.~Gruendl,True,"National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA",
Gschwend,Julia,julia@linea.gov.br,J.~Gschwend,True,"Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil",
Gschwend,Julia,julia@linea.gov.br,J.~Gschwend,True,"Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil",
Gutierrez,Gaston,gaston@fnal.gov,G.~Gutierrez,True,"Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA",0000-0003-0825-0517
Hollowood,Devon L.,dhollowo@ucsc.edu,D.~L.~Hollowood,True,"Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA",
James,David,djames44@gmail.com,D.~J.~James,True,"Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA}",
Jeltema,Tesla,tesla@ucsc.edu,T.~Jeltema,True,"Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA",
Kuehn,Kyler,kkuehn@aao.gov.au,K.~Kuehn,True,"Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia",0000-0003-0120-0808
Lima,Marcos,mlima@if.usp.br,M.~Lima,True,"Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil",
Lima,Marcos,mlima@if.usp.br,M.~Lima,True,"Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil",
Maia,Marcio,maia@fnal.gov,M.~A.~G.~Maia,True,"Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil",
Maia,Marcio,maia@fnal.gov,M.~A.~G.~Maia,True,"Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil",
Marshall,Jennifer,jlm076@tamu.edu,J.~L.~Marshall,True,"George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA",0000-0003-0710-9474
Martini,Paul,martini.10@osu.edu,P.~Martini,True,"Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA",0000-0002-4279-4182
Martini,Paul,martini.10@osu.edu,P.~Martini,True,"Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA",0000-0002-4279-4182
Melchior,Peter,peter.m.melchior@gmail.com,P.~Melchior,True,"Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA",
Menanteau,Felipe,felipe@illinois.edu,F.~Menanteau,True,"Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA",0000-0002-1372-2534
Menanteau,Felipe,felipe@illinois.edu,F.~Menanteau,True,"National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA",0000-0002-1372-2534
Miller,Christopher,christoq@umich.edu,C.~J.~Miller,True,"Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA",
Miller,Christopher,christoq@umich.edu,C.~J.~Miller,True,"Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA",
Miquel,Ramon,rmiquel@ifae.es,R.~Miquel,True,"Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain",0000-0002-6610-4836
Miquel,Ramon,rmiquel@ifae.es,R.~Miquel,True,"Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain",0000-0002-6610-4836
Ogando,Ricardo,ogando@on.br,R.~L.~C.~Ogando,True,"Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil",0000-0003-2120-1154
Ogando,Ricardo,ogando@on.br,R.~L.~C.~Ogando,True,"Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil",0000-0003-2120-1154
Plazas Malag처n,Andr챕s,plazasmalagon@gmail.com,A.~A.~Plazas,True,"Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA",0000-0002-2598-0514
Sanchez,Eusebio,eusebio.sanchez@ciemat.es,E.~Sanchez,True,"Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain",0000-0002-9646-8198
Scarpine,Vic,scarpine@fnal.gov,V.~Scarpine,True,"Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA",
Schubnell,Michael,schubnel@umich.edu,M.~Schubnell,True,"Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA",
Serrano,Santiago,serrano@ieec.uab.es,S.~Serrano,True,"Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain",
Serrano,Santiago,serrano@ieec.uab.es,S.~Serrano,True,"Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain",
Sevilla,Ignacio,nsevilla@fnal.gov,I.~Sevilla-Noarbe,True,"Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain",
Smith,Mathew,mat.smith@soton.ac.uk,M.~Smith,True,"School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK",0000-0002-3321-1432
Soares-Santos,Marcelle,marcelle@fnal.gov,M.~Soares-Santos,True,"Brandeis University, Physics Department, 415 South Street, Waltham MA 02453",0000-0001-6082-8529
Sobreira,Flavia,sobreira@linea.gov.br,F.~Sobreira,True,"Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil",0000-0002-7822-0658
Sobreira,Flavia,sobreira@linea.gov.br,F.~Sobreira,True,"Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil",0000-0002-7822-0658
Suchyta,Eric,eric.d.suchyta@gmail.com,E.~Suchyta,True,"Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831",0000-0002-7047-9358
Swanson,Molly,molly.swanson@gmail.com,M.~E.~C.~Swanson,True,"National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA",
Tarle,Gregory,gtarle@umich.edu,G.~Tarle,True,"Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA",0000-0003-1704-0781
Thomas,Daniel,daniel.thomas@port.ac.uk,D.~Thomas,True,"Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK",
Weller,Jochen,jochen.weller@usm.lmu.de,J.~Weller,True,"Excellence Cluster Origins, Boltzmannstr.\ 2, 85748 Garching, Germany",0000-0002-8282-2010
Weller,Jochen,jochen.weller@usm.lmu.de,J.~Weller,True,"Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany",0000-0002-8282-2010
Weller,Jochen,jochen.weller@usm.lmu.de,J.~Weller,True,"Universit\""ats-Sternwarte, Fakult\""at f\""ur Physik, Ludwig-Maximilians Universit\""at M\""unchen, Scheinerstr. 1, 81679 M\""unchen, Germany",0000-0002-8282-2010


==> authorlist.tex <==
% Author list file generated with: mkauthlist 1.2.3+16.gfd56256 
% mkauthlist --sort-builder ../DMASS-paper/authorlist ../DMASS-paper/authorlist.tex 

\author{S.~Lee}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Department of Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{A.~Choi}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{C.~Davis}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\author{T.~F.~Eifler}
\affiliation{Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\author{K.~Honscheid}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Department of Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{E.~M.~Huff}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\author{N.~MacCrann}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Department of Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{A.~J.~Ross}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{M.~A.~Troxel}
\affiliation{Department of Physics, Duke University Durham, NC 27708, USA}
\author{J.~Annis}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{S.~Avila}
\affiliation{Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain}
\author{D.~Brooks}
\affiliation{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\author{A.~Carnero~Rosell}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{M.~Carrasco~Kind}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{J.~Carretero}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain}
\author{R.~Cawthon}
\affiliation{Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390}
\author{L.~N.~da Costa}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{J.~De~Vicente}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{S.~Desai}
\affiliation{Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India}
\author{B.~Flaugher}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{P.~Fosalba}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain}
\author{J.~Garc\'ia-Bellido}
\affiliation{Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain}
\author{E.~Gaztanaga}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain}
\author{D.~W.~Gerdes}
\affiliation{Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{D.~Gruen}
\affiliation{Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA}
\affiliation{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\author{R.~A.~Gruendl}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{J.~Gschwend}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{G.~Gutierrez}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{D.~L.~Hollowood}
\affiliation{Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA}
\author{D.~J.~James}
\affiliation{Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA}}
\author{T.~Jeltema}
\affiliation{Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA}
\author{K.~Kuehn}
\affiliation{Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia}
\author{M.~Lima}
\affiliation{Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{M.~A.~G.~Maia}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{J.~L.~Marshall}
\affiliation{George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA}
\author{P.~Martini}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA}
\author{P.~Melchior}
\affiliation{Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA}
\author{F.~Menanteau}
\affiliation{Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{C.~J.~Miller}
\affiliation{Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{R.~Miquel}
\affiliation{Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain}
\affiliation{Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain}
\author{R.~L.~C.~Ogando}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\affiliation{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{A.~A.~Plazas}
\affiliation{Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA}
\author{E.~Sanchez}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{V.~Scarpine}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{M.~Schubnell}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{S.~Serrano}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain}
\affiliation{Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain}
\author{I.~Sevilla-Noarbe}
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\author{M.~Smith}
\affiliation{School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK}
\author{M.~Soares-Santos}
\affiliation{Brandeis University, Physics Department, 415 South Street, Waltham MA 02453}
\author{F.~Sobreira}
\affiliation{Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil}
\affiliation{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\author{E.~Suchyta}
\affiliation{Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831}
\author{M.~E.~C.~Swanson}
\affiliation{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\author{G.~Tarle}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{D.~Thomas}
\affiliation{Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK}
\author{J.~Weller}
\affiliation{Excellence Cluster Origins, Boltzmannstr.\ 2, 85748 Garching, Germany}
\affiliation{Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany}
\affiliation{Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany}


\collaboration{(DES Collaboration)}


==> constraints.tex <==
\section{Cosmological Constraints}
\label{sec:constraints}
\notesj{$\sigma_8$ - $\Omega_m$ in $\Lambda CDM$}



==> redshift.tex <==
\subsection{Redshift Distribution}

%\cmt{Why redshift distribution is important}
%Photometric redshift is inaccurate. DES photometric redshift is derived from DES colors. Therefore, it conveys various of combination of DES photometric errors. Its error reaches [..]. and DMASS photometric redshift is biased by ( ) compared to CMASS spectroscopic redshift. Our extreme deconvolution model is selecting galaxies based on their photometric color sets, thus even if the resulted galaxy sample has the same photometric redshift as the train sample it may not have the same true redshift distribution. 


%\cmt{introducing clsutering reshift distribution}
In this section, we evaluate the redshift distribution of the DES-CMASS sample by cross-correlating DES-CMASS galaxies with the DES \redmagic sample \citep{Rozo2016RedMaGiC:Data}. 
The concept of this technique called 'clustering-z' is to recover redshift distributions of an unknown sample by cross-correlating it with a galaxy sample whose redshift distribution is known and accurate.
The technique was first studied in \cite{Schneider2006CrossCorrelation}, and has been developed and applied to various cosmological analyses including DES \citep{2016MNRAS.460..163R,2016MNRAS.463.3737C,2017MNRAS.465.4118J,2017MNRAS.467.3576M,2018MNRAS.474.3921S}. 
%This method is referred to 'clustering-z' and 
%originally intended to cross-correlate a spectroscopic sample with an unknown sample that one wants to evaluate redshift distributions as \cite{Cawthon2017DarkCross-Correlations}
%One can also use photometric redshifts in the same manner, given that they are accurate and the redshift distribution that one wishes to characterize is broad \citep{Gatti2018}.
%using spectroscopic sample as a reference sample, 
\cite{Gatti2018} and \cite{Davis2017} calibrated redshift distributions of the DES Y1 source samples by using the DES \redmagic \citep{Rozo2016RedMaGiC:Data} as a reference sample. 
\cite{Cawthon2017DarkCross-Correlations} calibrated the DES \redmagic sample by cross-correlating with the BOSS spectroscopic galaxy samples. For further details about the clustering-z method, we refer interested readers to references in \cite{Cawthon2017DarkCross-Correlations}. 
%The reference sample in their work is the DES redmagic high luminosity sample \REF{REF:ROZO et al}
%as a reference sample to calibrate the redshift distributions of the DES Y1 source sample. 

We utilized the \redmagic sample as a reference sample and followed the general procedures described in \cite{Davis2017}. 
The \redmagic sample is made of red luminous galaxies above some minimal luminosity threshold selected by the redMaPPer algorithm \citep{Rykoff2014RedMaPPer.Catalog}. These galaxies have excellent photometric redshifts with an approximately Gaussian scatter of $\sigma_z/(1+z) < 0.02$ and cover the entire DES Y1 footprint. This makes them suitable as a reference sample to evaluate the redshift distribution of DES-CMASS sample.
We chose the higher luminosity \redmagic sample selected above a luminosity threshold of $L > 1.5L_*$.
%along with the same comoving scale cuts from $500 \kpc$ to $1500 \kpc$. 
%unlike spectroscopic samples over a minimal area \REF{ROZO} which makes them suitable for a reference sample even though they don't have spectroscopic redshifts. 
%The DES redmagic sample doesn't have the spectroscopic redshift but its photometric redshift is accurate at the level of $sigma < 0.2$(?) \REF{REF: ROZO}. Also DES redmagic sample has more galaxies than any other spectroscopic sample existing in the DES Y1 footprint. 
%From the DES Y1 Gold Catalog we select a subset of objects using the redMaGiC algorithm (Rozo et al. 2016). The algorithm aims to define a sample of luminous red galaxies above some minimal luminosity threshold. These galaxies are selected by fitting to a red sequence template that was calibrated using galaxy clusters selected by the redMaPPer algorithm (Rykoff et al. 2014, 2016). These galaxies are selected to have a constant comoving number density of galaxies as a function of redshift, and have excellent photo-z’s, with an approximately Gaussian scatter of σz/(1 + z) < 0.02 (Rozo et al. 2016). The high quality of the redMaGiC pho- tometric redshifts makes them an appropriate sample for measuring

%To measure the true redshift distribution of DMASS, we use the clustering-z technique described in \REF{Getti et al, Cawthon et al, Davis et al}. 

%Getti et al suggested to use cross correlation function between unknown sample and reference spectroscopic sample to constrain redshift distribution of unknown sample. 
%Cawthon et al constrained redshift distribution of full BOSS CMASS sample by cross-correlating it with redmagic spectroscopic sample in the SDSS footprint. 
%Unlike previous studies using spectroscopic sample as a reference sample, Davis et al used photometric galaxy sample for the first time. They used the DES redmagic high luminosity sample[REF:ROZO et al] as a reference sample to calibrate the redshift distributions of the DES Y1 source sample. The DES redmagic sample doesn't have the spectroscopic redshift but its photometric redshift is very accurate at the level of $sigma < 0.2$(?) [REF: ROZO]. Also DES redmagic sample has more galaxies than any other spectroscopic sample existing in the DES Y1 footprint. 

%\cmt{simple theory}

To obtain the redshift distribution of the unknown sample, we split the reference sample in narrow redshift bins, $\Delta z = 0.02$, and measure cross-correlations between the galaxies in each redshift bin and the unknown sample. This cross-correlation for $i$th redshift bin is given as
%for each subsample i we measure its angular or spa- tial correlations with the unknown population
\bea
w^{ur}(z_i) = \int^{R_{\rm max}}_{R_{\rm min}} \ud R~ \ud z' ~b^u(z') b^r(z_i) 
\label{eq:wur} \\
\times ~ n^u(z') n^r(z_i) \xi_m (R, z_i, z') 
\nonumber
\eea
where $b$ denote galaxy bias of the unknown('u') and reference('r') sample, $n(z)$ stands for a normalized redshift distribution, $\xi_m$ stands for matter clustering. $z_i$ is $i$th redshift bin of the reference sample. $R$ is comoving distance, $R = (1+z) D_A(z) \theta$. 
%\reph{The method counts unknown galaxies in annuli around each reference galaxy bounded by comoving distance $R = (1+z) D_A \theta$ from $R_{\rm min}$ to $R_{\rm max}$. } 
We adopt $R_{\rm min} = 500 \kpc$ and $R_{\rm max} = 1500 \kpc$ based on \cite{Gatti2018} and \cite{Davis2017}. %\cite{Gatti2018} demonstrated that in simulation clustering-z is largely scale-independent, with a decrease in signal-to-noise at larger scales. 
We also assume that galaxy biases of both the reference and unknown sample are scale-independent on these scales.  \cite{Schmidt2013RecoveringBoundaries} demonstrated that implementing a linear bias model in the clustering-z does not significantly impact on the methodology, even if these scales are non-linear. The same point was made in \cite{Gatti2018} and \cite{Cawthon2017DarkCross-Correlations} as well. For narrow redshift bins $n^r(z_i) = \delta(z-z_i)$, equation \ref{eq:wur} is simplified as 
\bea
w^{ur}(z_i) = n^u(z_i) b^u(z_i)  b^r(z_i) \bar{w}_m(z_i)
\eea
where $\bar{w}_m$ is the integrated correlation function between $R_{\rm min}$ and $R_{\rm max}$. 
The cross-correlation was measured with the estimator from \cite{DavisPeebles1983} as follow:
%We use the estimator from \REF{DavisPeebles1983} to measure cross-correlations as follow:
\bea
\hat{w}^{ur}(z) = \frac{N_{R^r}}{{N_{D^r}}} \frac{ \int^{R_{\rm max}}_{R_{\rm min}}  \ud R ~W(R) [D^u D^r(R,z)] }{ \int^{R_{\rm max}}_{R_{\rm min}} \ud R~ W(R) [D^u R^r(R,z)] }-1 
\eea
where $W(R)$ is a weighting function, $D_u D_r$ and $D_u R_r$ stand for the number of galaxy-galaxy and galaxy-random pairs, $N_{R^r}$ and $N_{D^r}$ stand for the total number of randoms and galaxies of the reference sample. With the measured cross correlation, the redshift distributions of the unknown sample is given as 
\bea
n^u (z) \propto \frac{\hat{w}^{ur} (z) }{ b^u(z) b^r (z) \bar{w}_m(z) }.
\eea
The galaxy bias evolution of the reference sample $b^r$ can be obtained from the measured auto correlation of the reference sample as follow
\bea
\hat{w}^{rr}(z) = [b^r(z)]^2 \bar{w}_m (z).
\eea
For galaxy bias of the unknown sample, we adopt $b^u = 2$ ignoring redshift evolution as the galaxy bias of CMASS is nearly constant within its redshift range $0.4 < z < 0.7$, and we expect our selection to match.
%\cmt{our work}
%We followed general procedures described in \cite{Davis2017}. We chose the high luminosity \redmagic sample selected above a luminosity threshold of $L > 1.5L_*$ along with the same comoving scale cuts from $500 \kpc$ to $1500 \kpc$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Description about luminosity cut : there are three different redmagic sample; high density, high luminosity, higher luinosity. DES chose different samples depending on the redshift range the lens sample covers. Davis et al 2017 showed that combining all three samples and using only one kind of sample yield almost the same result, so decided to use only one sample - higher luminosity - to make the case simple, and also reduce the potential systematics. 
% Description about scale choice : Large scales have full SNR. On small scales, we expected that on data the smaller scales would become suspect because of issues like deblending which were not modeled in the simulations. Also Gatti2017 showed that in simulation clustering-z is largely scale-indelendent, with a decrease in SNR at larger scales. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The clustering redshift method requires a model of the galaxy bias for the target sample. The galaxy bias of CMASS is a nearly constant ($b=2$) within the redshift range $0.4 < z < 0.7$ \REF{CMASS bias}, and we expect our selection to match. 

%\reph{ However, a small fraction of the CMASS sample has $z < 0.4$ (see Fig. 10) and part of this test is to determine how much of the DES-CMASS sample has $z<0.4$. It is possible, for instance, that the probabilistic model is prone to select slightly more galaxies near the $\dperp$ cut and that this would cause  DES-CMASS to include more galaxies at low redshift than CMASS. We do not know, a priory, the bias of these galaxies that are essentially contaminants. To account for this we choose a varying galaxy bias model that gradually increases starting from a lower galaxy bias $b=1$ at $z=0$ that smoothly evolves to $b=2$ at $z=0.4$ as $b(z) = z/0.4 + 1$, and is constant for $z>0.4$. We also tested a constant galaxy bias over full redshift range and obtained consistent results {\bf it might be nice to show this as well}. We conclude that our results are robust to the assumed galaxy bias.}

Fig. \ref{fig:dmass_nz} shows the result obtained from clustering-z. We find an excellent agreement between the clustering redshift distribution of DES-CMASS (blue points with error bars) and the spectroscopic redshift of CMASS SGC (solid black curve). The $\chi^2$ obtained when comparing the two is $34$ for 36 data points. We conclude that the clustering redshift method returns a $n(z)$ for DES-CMASS that is consistent with the BOSS SGC $n(z)$. 
%The error bars are calculated from [...] 
%We obtained a derived redshift distribution with an excellent agreement at high redshift, with a $\chi^2 / dof$ value of $26.1/36$. 
%

%The redshift distribution shows a little bump at $z \sim 0.4$ where $\dperp$ cut is located. This is expected as the probabilistic model tends to select more galaxies near the noisy $\dperp$ cut. In spite of the little disagreement, the $\chi^2$ value less than $1$ implies the redshift distribution of DES-CMASS is effectively same with the CMASS spectroscopic redshift. 
%{\bf I think I would remove this paragraph...the points are not overly significant and if they were they might not even have anything to do with DMASS (could be redmagic) }\sjcmt{ We don't have evidence that this is because of redmagic and ppl would question that bump as soon as they see the plot}

%The redshift distribution shows a less agreement at $z \sim 0.4$ where the extreme deconvolution model suffers low probability casued by large SDSS photometric errors and filter difference at the g-r transition.
%\cmt{the effect of a bump at $z \sim 0.4$}
%We tested bias evolution model in case the little bump at $z\sim 0.4$ is caused by over estimated galaxy bias of galaxies at low redshift.\\



\subsection{ Error on galaxy bias and other cosmological parameters}
\label{sec:result-bias}

In this section, we present the constraint of galaxy bias of the DES-CMASS sample derived from the results of auto angular clustering and clustering redshift distribution in the previous section. 
Auto angular clustering computed in the previous section shows sufficient signal to noise  to constrain galaxy bias strongly, but galaxy bias is degenerate with the uncertainty of the redshift distribution leading to weaker constraints than DES-CMASS is supposed to achieve. Thus, we utilize the clustering-z distribution of DES-CMASS obtained independently from the auto angular clustering to constrain the uncertainty of redshift distribution. 



%From the previous section, we measured the true redshift distribution of DES-CMASS with the excellent $\chi^2$ value against the CMASS spectroscopic redshift. 
%There is no doubt that the shape of CMASS spec-z distribution is a good model for DES-CMASS redshift distribution. 
%However, the clustering-z method works under the assumption that DES-CMASS galaxy bias is perfectly linear and same with CMASS galaxy bias. Since galaxy bias is degenerated with redshift distribution, a small shift in galaxy bias would result in a bias in redshift distribution. 


%To marginalize the uncertainty of the redshift distribution, we introduced a redshift bin bias parameter $\Delta z$ that goes into the redshift distribution function as an additive parameter as $n(z_i + \Delta z)$. 

%With a covariance matrix obtained from the previous section, we constrained the redshift bias $\Delta z$ using a CMASS redshift distribution as a fiducial data vector with no assumption about galaxy bias.



%Auto angular clustering has both galaxy bias and redshift distribution, and also we obtained a good agreement at this. Therefore, using angular clustering to constrain the shifts in both galaxy bias and redshift distribution is the most reasonable way we can try.

The model of angular clustering is
\bea
\omega_g(\theta) = \int \ud z ~(b_g+\Delta b_g)^2 ~ n_g(z + \Delta z)^2 ~\xi_m (\chi\theta, z)
\eea
where $\xi_m$ is the matter angular clustering, $\Delta b$ and $\Delta z$ imply a shift in galaxy bias and the redshift distribution from fiducial quantities. Those parameters are set to zero for CMASS. 
%from the galaxy bias of CMASS SGC or full CMASS, and $\Delta z$ is a shift in the redshift distribution $n(z)$ from values of CMASS galaxies. 
We ignore galaxy bias evolution as function of redshift because 1. CMASS galaxy bias barely evolves with respect to redshift, 2. The redshift range from 0.4 to 0.7 is narrow enough to ignore the effect of galaxy bias evolution, especially for galaxy clustering.
%To perform a likelihood analysis, we determined residuals of angular clusterings as a data vector as
%\bea
%d = w_g^{\rm DES-CMASS} (\theta) - w_g^{\rm CMASS} (\theta)~.
%- [w_g^{\rm DES-CMASS, model} (\theta) - w_g^{\rm CMASS, model} (\theta)] .
%\eea
%We adopt $\Delta b =0$ and $\Delta z = 0$ for CMASS samples. 
%The fiducial value of galaxy bias for the model is $b=2$.
We performed a likelihood analysis with the measurements and theoretical models as follow:
\bea
\chi^2 = ( d - d^T ) ~ C^{-1} ~ ( d - d^T ),
\eea
where the data vector $d$ is the residuals between measurements of angular clustering of DES-CMASS and CMASS in SGC or full CMASS, and $d^T$ stands for the residuals of the models, $\Delta w(\theta) = w(\theta) - w(\theta, \Delta b, \Delta z)$, where $\Delta b$ and $\Delta z$ are free parameters.
The covariance matrix is given as the sum of jackknife covariance matrix obtained from auto angular clustering as
\bea
C = C_{\rm DES-CMASS} + C_{\rm CMASS}~.
\eea

We also constrained $\Delta z$ separately using the covariance matrix and the inferred redshift distribution of DES-CMASS obtained in the previous section. The spectroscopic redshift distributions of CMASS SGC and full CMASS are used as true values with the following equation:
\bea
\chi^2 = (n_{\rm spec}(z) - n(z+\Delta z)) ~C_{z}^{-1}~ (n_{\rm spec}(z) - n(z+\Delta z)),
\nonumber
\eea
where $C_z$ is the covariance matrix obtained from the clustering-z calculation in the previous section.
%The resulting $\Delta z$ shows $\Delta z = 0.0^{+0.005}_{-0.005}$ for CMASS SGC as a fiducial sample. 

%To marginalize the uncertainty of the redshift distribution, we introduced a redshift bin bias parameter $\Delta z$ that goes into the redshift distribution function as an additive parameter as $n(z_i + \Delta z)$. 

%With a covariance matrix obtained from the previous section, we constrained the redshift bias $\Delta z$ using a CMASS redshift distribution as a fiducial data vector with no assumption about galaxy bias.

%We only adopt scales from \cmt{0.0} arcmin to \cmt{0.0} arcmin to ensure the scales where linear galaxy bias theory is valid. 
Figure \ref{fig:bias_final} shows bias shift and redshift shift from each fiducial samples and combination with clutering-z. 
%<<<<<<< sharelatex-2018-12-07-2329
%Blue and black contours show the constraints of galaxy bias shift from CMASS SGC and full CMASS, respectively when the redshift distribution is marginalized. The extremely stretched contours imply that that uncertainties of galaxy bias and redshift distribution are strongly degenerated, thereby extra information should be needed to break the degeneracy. The green contour is only constraining $\Delta z$ with DES-CMASS clustering-z. The resulting $\Delta z$ shows $\Delta z = \dzonly$ for CMASS SGC as a fiducial sample. 
%The red and orange contours show the combination of the two probes, angular clustering and clustering-z. The resulting numbers for DES-CMASS are $\Delta b = \dbsgc$ and $\Delta z = \dzsgc$ against CMASS SGC, and $\Delta b = \dbfull$ and $\Delta z = \dzfull$ against full CMASS. As expected, DES-CMASS achieves a better agreement with CMASS in SGC but keep $1\sigma$ deviations for both cases, despite angular clustering comparison with full CMASS is the one showing the least agreement among all comparison tests performed in this paper. The resulted bias deviation is less than $5\%$ for both cases which is safely below the error budget of CMASS galaxy bias $10\%$ with a combination of the structrue growth rate $f$ \citep{Chuang2017} and also smaller than the intrinsic difference of galaxy bias between CMASS SGC and CMASS NGC shown in appendix \ref{app:ngc_sgc}.
%=======
Blue and black contours show the constraints of galaxy bias shift from CMASS SGC and full CMASS respectively when the redshift distribution is marginalized. The extremely stretched contours imply that that uncertainties of galaxy bias and redshift distribution are strongly degenerated, thereby extra information should be needed to break the degeneracy. The green contour is only constraining $\Delta z$ with DES-CMASS clustering-z. The resulting $\Delta z$ shows $\Delta z = \dzonly$ for CMASS SGC as a fiducial sample. 
The red and orange contours show the combination of the two probes, angular clustering and clustering-z. The resulting numbers for DES-CMASS are $\Delta b = \dbsgc$ and $\Delta z = \dzsgc$ against CMASS SGC, and $\Delta b = \dbfull$ and $\Delta z = \dzfull$ against full CMASS. As expected, DES-CMASS achieves a better agreement with CMASS in SGC but keep $1\sigma$ deviations for both cases, despite angular clustering comparison with full CMASS is the one showing the least agreement among all comparison tests performed in this paper. The resulted bias deviation is less than $5\%$ for both cases which is safely below the error budget of CMASS galaxy bias $10\%$ with a combination of the structure growth rate $f$ \citep{Chuang2017} and also comparable to $5\%$ of the intrinsic difference of galaxy bias between CMASS SGC and CMASS NGC shown in appendix \ref{app:ngc_sgc}.
%>>>>>>> master


%{\bf AJR didn't do anything in this section, will wait until it is more complete}

%Goal : bias of DMASS sample (obtained from ggl) should be within error budget of CMASS cl + planck when the uncertainty of lowz fraction is marginalized.
%\bea
%b_{CMASS,cl} - b_{DMASS,ggl} < \sigma_{b, planck + CMASS}
%\eea





\begin{figure}
%\includegraphics[width=0.6\textwidth]{./figures/dmass_spt_deviation}
% (CMH) commented out so this will compile
\centering
\includegraphics[width=0.5\textwidth]{./figures/nz.pdf}
\caption{ Redshift distribution of DES-CMASS (blue) recovered by the  clustering-z method with \redmagic. The solid black and dashed lines show the spectroscopic redshift distribution of CMASS SGC and full CMASS. The value of $\chi^2/{\rm dof}$ obtained against CMASS SGC is less than 1.0 
	 }
\label{fig:dmass_nz}
\end{figure}

\begin{figure}
%\includegraphics[width=0.6\textwidth]{./figures/dmass_spt_deviation}
% (CMH) commented out so this will compile
\centering
\includegraphics[width=0.45\textwidth]{./figures/emcee_bias_nz.pdf}
\caption{ Constraints of galaxy bias shift $\Delta b$ and redshift distribution shift $\Delta z$ from various data sets. The dashed line shows the ideal case where DES-CMASS is perfectly matched with CMASS. Because of the strong degeneracy between galaxy bias and redshift distribution, angular clustering only shows extremely stretched contours in the diagonal direction. Adding clustering-z breaks the degeneracy and resulted in $\Delta b = \dbsgc$ for CMASS SGC (red) and $\Delta b = \dbfull$ for full CMASS (orange). The uncertainty of the galaxy bias shift for CMASS SGC is $\sigma_{\Delta b} \sim 0.08$, which is about $4\%$ of the fiducial value.}
\label{fig:bias_final}
\end{figure}

